Unified Algorithms for RL with Decision-Estimation Coefficients: PAC, Reward-Free, Preference-Based Learning, and Beyond

Modern Reinforcement Learning (RL) is more than just learning the optimal policy; Alternative learning goals such as exploring the environment, estimating the underlying model, and learning from preference feedback are all of practical importance. While provably sample-efficient algorithms for each specific goal have been proposed, these algorithms often depend strongly on the particular learning goal and thus admit different structures correspondingly. It is an urging open question whether these learning goals can rather be tackled by a single unified algorithm. We make progress on this question by developing a unified algorithm framework for a large class of learning goals, building on the Decision-Estimation Coefficient (DEC) framework. Our framework handles many learning goals such as no-regret RL, PAC RL, reward-free learning, model estimation, and preference-based learning, all by simply instantiating the same generic complexity measure called "Generalized DEC", and a corresponding generic algorithm. The generalized DEC also yields a sample complexity lower bound for each specific learning goal. As applications, we propose "decouplable representation" as a natural sufficient condition for bounding generalized DECs, and use it to obtain many new sample-efficient results (and recover existing results) for a wide range of learning goals and problem classes as direct corollaries. Finally, as a connection, we re-analyze two existing optimistic model-based algorithms based on Posterior Sampling and Maximum Likelihood Estimation, showing that they enjoy sample complexity bounds under similar structural conditions as the DEC.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preamble-ams.tex <==
\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %



\usepackage{amsmath}
\usepackage{amsxtra,amsfonts,amscd,amssymb,bm,bbm,mathrsfs}
\usepackage{nicefrac}       %
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{mathabx}

\usepackage[algo2e,linesnumbered,vlined,ruled]{algorithm2e}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\usepackage{url}
\usepackage{breakcites}
\usepackage[usenames,dvipsnames]{color}
\hypersetup{
  colorlinks,
  citecolor=blue!70!black,
  linkcolor=blue!70!black,
  urlcolor=blue!70!black
}
\usepackage[capitalise]{cleveref}
\usepackage[titletoc,title]{appendix}
\usepackage{cancel}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{comment}
\crefformat{equation}{#2(#1)#3}
\Crefformat{equation}{#2(#1)#3}


\usepackage{booktabs}       %
\usepackage{multirow}
\usepackage{multicol}
\usepackage{makecell}
\usepackage{array}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\newcolumntype{Z}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{\hspace*{-\tabcolsep}}}

\usepackage[normalem]{ulem}
\usepackage{exscale}
\usepackage{tikz}
\usepackage{float}
\usepackage{graphicx,graphics}
\graphicspath{ {./fig/} }
\allowdisplaybreaks


\newenvironment{proofof}[1][{}]{\noindent{\emph{Proof of \cref{#1}.}}
  \hspace*{1em}}{\qed\bigskip\\}


\newcommand{\comm}[1]{{\color{red}#1}}
\newcommand{\revise}[1]{{#1}}
\newcommand{\remove}[1]{{\color{Gray}\sout{#1}}}

\def\shownotes{0}  %
\ifnum\shownotes=0
\newcommand{\authnote}[2]{{\scriptsize $\ll$\textsf{#1 notes: #2}$\gg$}}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\yub}[1]{{\color{red}\authnote{Yu}{#1}}}
\newcommand{\cfn}[1]{{\color{blue}\authnote{cf}{#1}}}
\newcommand{\sm}[1]{{\color{blue}\authnote{Song}{#1}}}

\newcommand{\todo}[1]{{\color{blue}$\ll$\textsf{\footnotesize TODO:
      {#1}$\gg$}}}
      
\renewcommand{\hat}{\widehat}
\renewcommand{\epsilon}{\varepsilon}

\usepackage{pifont}
\newcommand{\no}{\ding{55}}
\newcommand{\yes}{\ding{51}}
\newcommand{\id}{I}
\newcommand{\tA}{\tilde{\mathcal{A}}} 
\newcommand{\tC}{\tilde{C}}  
\newcommand{\tX}{\tilde{X}}    
\newcommand{\tZ}{\tilde{Z}} 
\newcommand{\tM}{\tilde{M}}
\newcommand{\nS}{|\mathcal{S}|}
\newcommand{\nA}{|\mathcal{A}|}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Eps}{\mathcal{E}}
\newcommand{\hX}{X}
\newcommand{\hY}{Y}
\newcommand{\hZ}{Z}
\newcommand{\II}{\mathbb{I}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\DD}{\mathbb{D}}
\newcounter{cnt}
\setcounter{cnt}{0}
\foreach \num in {1,2,...,26}{%
  \stepcounter{cnt}%
  \expandafter\xdef \csname c\Alph{cnt}\endcsname {\noexpand\mathcal{\Alph{cnt}}}%
  \expandafter\xdef \csname b\Alph{cnt}\endcsname {\noexpand\mathbb{\Alph{cnt}}}%
}
\renewcommand{\bR}{\mathbf{R}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\im}{\operatorname{Im}}
\newcommand{\ind}{\mathrm{1}}
\newcommand{\sgn}{\mathrm{sgn}} 
\newcommand{\spa}{\mathrm{span}} 
\newcommand{\orth}{\mathbf{orth}} 
\newcommand{\prox}{\mathbf{prox}} 
\newcommand{\ket}[1]{\left\vert{#1}\right\rangle}
\newcommand{\bra}[1]{\left\langle{#1}\right\vert}
\newcommand{\braket}[2]{\left\langle{#1}\vert{#2}\right\rangle}
\newcommand{\dom}{\mathrm{dom}} 
\newcommand{\dist}{\mathrm{dist}} 
\newcommand{\ivec}{\mathrm{vec}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\diam}{diam}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\TV}{\operatorname{TV}}

\newcommand{\reg}{\mathbf{Reg}}
\newcommand{\regret}{\mathrm{regret}}
\newcommand{\violation}{\mathrm{violation}}
\newcommand{\mix}{\mathrm{mix}}

\newcommand{\verify}{\text{V\small{ERIFY}}}
\newcommand{\true}{\text{T\small{RUE}}}
\newcommand{\false}{\text{F\small{ALSE}}}

\newcommand{\leqsim}{\lesssim}
\newcommand{\geqsim}{\gtrsim}
\newcommand{\minimize}{\mathop{\textrm{minimize}}}
\newcommand{\maximize}{\mathop{\textrm{maximize}}}
\newcommand{\st}{\mathop{\textrm{s.t.}\ }}  
\newcommand{\T}{\top}  
\newcommand{\iprod}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\nrm}[1]{\left\|#1\right\|}
\newcommand{\minop}[1]{\min\left\{#1\right\}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\sqr}[1]{\left\|#1\right\|^2}
\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\epct}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\cond}[2]{\mathbb{E}\left[\left.#1\right|#2\right]}
\newcommand{\condP}[2]{\mathbb{P}\left(\left.#1\right|#2\right)}
\newcommand{\condV}[2]{\mathbb{V}\left[\left.#1\right|#2\right]}
\newcommand{\bigO}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\tbO}[1]{\widetilde{\mathcal{O}}\left(#1\right)}
\newcommand{\tbbO}[1]{\tilde{\mathcal{O}}\big(#1\big)}
\newcommand{\tbOm}[1]{\tilde{\Omega}\left(#1\right)}
\newcommand{\Om}[1]{\Omega\left(#1\right)}
\newcommand{\ThO}[1]{\Theta\left(#1\right)}
\newcommand{\ceil}[1]{\left\lceil #1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1\right\rfloor}
\DeclarePairedDelimiterX{\ddiv}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\KL}{\operatorname{KL}\ddiv}
\newcommand{\Dtwo}{\operatorname{D}_{\chi^2}\ddiv}
\newcommand{\pos}[1]{\left[#1\right]_{+}}
\newcommand{\hnabla}{\widehat{\nabla}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\Fil}{\mathfrak{F}}
\newcommand{\highprob}{with probability at least $1-\nicefrac{\delta}{10}$}
\newcommand{\highprobs}[1]{with probability at least $1-\nicefrac{\delta}{#1}$}
\newcommand{\Highprobs}[1]{With probability at least $1-\nicefrac{\delta}{#1}$}
\newcommand{\highprobdemo}{with probability at least $1-\delta$}

\newcommand{\clog}{\iota}
\newcommand{\dlog}{\log(1/\delta)}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\vecone}{\be}


\newcommand{\bu}{\mathbf{u}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bzero}{\mathbf{0}}


\newcommand{\oV}{\bar{V}}
\newcommand{\hV}{\hat{V}}
\newcommand{\opi}{\overline{\pi}}
\newcommand{\hpi}{\hat{\pi}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\tpi}{\tilde{\pi}}


\newcommand{\Algo}{\mathsf{Alg}}
\newcommand{\condPt}[2]{\mathbb{P}_{\theta}\left(\left.#1\right|#2\right)}
\newcommand{\condPb}[2]{\mathbb{P}_{\pi_b}\left(\left.#1\right|#2\right)}

\newcommand{\norm}[1]{\left\|{#1}\right\|} %
\newcommand{\lone}[1]{\norm{#1}_1} %
\newcommand{\ltwo}[1]{\norm{#1}_2} %
\newcommand{\linf}[1]{\norm{#1}_\infty} %
\newcommand{\lzero}[1]{\norm{#1}_0} %
\newcommand{\dnorm}[1]{\norm{#1}_*} %
\newcommand{\lfro}[1]{\left\|{#1}\right\|_{\sf Fr}} %
\newcommand{\lnuc}[1]{\left\|{#1}\right\|_*} %
\newcommand{\matrixnorm}[1]{\left|\!\left|\!\left|{#1}
  \right|\!\right|\!\right|} %
\newcommand{\opnorm}[1]{\norm{#1}_{\rm op}} %
\newcommand{\normbigg}[1]{\bigg\|{#1}\bigg\|} %
\newcommand{\normbig}[1]{\big\|{#1}\big\|} %
\newcommand{\normBig}[1]{\Big\|{#1}\Big\|} %
\newcommand{\lonebigg}[1]{\normbigg{#1}_1} %
\newcommand{\ltwobigg}[1]{\normbigg{#1}_2} %
\newcommand{\ltwobig}[1]{\normbig{#1}_2} %
\newcommand{\ltwoBig}[1]{\normBig{#1}_2} %
\newcommand{\linfbigg}[1]{\normbigg{#1}_\infty} %
\newcommand{\norms}[1]{\|{#1}\|} %
\newcommand{\matrixnorms}[1]{|\!|\!|{#1}|\!|\!|} %
\newcommand{\matrixnormbigg}[1]{\bigg|\!\bigg|\!\bigg|{#1}\bigg|\!\bigg|\!\bigg|} %
\newcommand{\lones}[1]{\norms{#1}_1} %
\newcommand{\ltwos}[1]{\norms{#1}_2} %
\newcommand{\linfs}[1]{\norms{#1}_\infty} %
\newcommand{\lzeros}[1]{\norms{#1}_0} %
\newcommand{\lambdamax}[1]{\lambda_{\max}({#1})}
\newcommand{\lambdamin}[1]{\lambda_{\min}({#1})}
\newcommand{\vmax}[1]{v_{\max}({#1})}
\newcommand{\vmin}[1]{v_{\min}({#1})}

\renewcommand{\cO}{\mathcal{O}}
\newcommand{\tO}{\widetilde{\cO}}
\newcommand{\wt}{\widetilde}
\newcommand{\indic}[1]{\mathbf{1}\left\{#1\right\}} %
\newcommand{\indics}[1]{1\{#1\}} %

\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}

\newcommand{\sign}{\operatorname{sign}}

\renewcommand{\bM}{\mathbf{M}}
\renewcommand{\bN}{\mathbf{N}}
\renewcommand{\bQ}{\mathbf{Q}}
\renewcommand{\bP}{\mathbf{P}}
\newcommand{\hbQ}{\widehat{\mathbf{Q}}}
\newcommand{\gbQ}{\widecheck{\mathbf{Q}}}
\newcommand{\hbP}{\widehat{\mathbf{P}}}
\newcommand{\gbP}{\widecheck{\mathbf{P}}}
\newcommand{\hth}{\hat{\theta}}
\newcommand{\ta}{\tilde{a}}

\newcommand{\otau}{\overline{\tau}}
\renewcommand{\II}{\mathbbm{1}}




\newcommand{\setto}{\leftarrow}

\newcommand{\bd}{\mathbf{d}}
\newcommand{\unif}{{\rm Unif}}
\newcommand{\distH}[1]{d_\mathrm{H}\left( #1\right)}

\newcommand{\Bs}{\B^\star}
\newcommand{\bs}{\b^\star}
\newcommand{\bds}{\bd^\star}

\newcommand{\Model}{\mathfrak{M}}
\newcommand{\otheta}{\bar{\theta}}

\newcommand{\nM}{O^{m}A^{m-1}}

\newcommand{\hM}{\widehat{M}}
\renewcommand{\hV}{\widehat{V}}
\newcommand{\oM}{{\overline{M}}}
\newcommand{\omu}{\overline{\mu}}

\newcommand{\dec}{\operatorname{dec}}
\newcommand{\psc}{\operatorname{psc}}
\newcommand{\omlec}{\operatorname{mlec}}
\newcommand{\mlec}{\operatorname{mlec}}
\newcommand{\odec}{\dec}
\newcommand{\eec}{\operatorname{pacdec}}
\newcommand{\oeec}{\eec}
\newcommand{\oeecg}{\oeec_{\gamma}}
\newcommand{\eecg}{\operatorname{edec}_{\gamma}}
\newcommand{\pscest}{\psc^{\exp}}
\newcommand{\pscestg}{\pscest_{\gamma}}
\newcommand{\dcpl}{\mathrm{dc}}

\newcommand{\obs}{\operatorname{obs}}
\newcommand{\rew}{\operatorname{rew}}
\newcommand{\dH}{D_{\mathrm{H}}}
\newcommand{\dTV}{D_{\mathrm{TV}}}
\newcommand{\wtdH}{D_{\operatorname{RL}}}
\renewcommand{\DH}[1]{D_{\mathrm{H}}^2\left(#1\right)}
\newcommand{\tDH}[1]{D_{\mathrm{RL}}^2\left(#1\right)}
\newcommand{\DTV}[1]{D_{\mathrm{TV}}\left(#1\right)}
\newcommand{\DTVt}[1]{D_{\mathrm{TV}}^2\left(#1\right)}

\newcommand{\subopt}{\mathbf{SubOpt}}

\newcommand{\co}{\operatorname{co}}
\newcommand{\regdm}{\mathbf{Reg}_{\mathbf{DM}}}
\newcommand{\dimbe}{\operatorname{dim}_{\rm BE}}
\newcommand{\eluder}{\mathfrak{e}}
\newcommand{\starn}{\mathfrak{s}}
\newcommand{\est}{\operatorname{Est}}
\newcommand{\Alg}{\mathbf{Alg}}
\newcommand{\Est}{\mathbf{Est}}
\newcommand{\EstwtH}{\mathbf{Est}_{\operatorname{RL}}}
\newcommand{\EstRL}{\mathbf{Est}_{\operatorname{RL}}}

\newcommand{\EstH}{\mathbf{Est}_{\mathrm{H}}}
\newcommand{\fl}{\operatorname{fl}}

\newcommand{\Ms}{{M^{\star}}}
\newcommand{\Vs}{V_\star}

\newcommand{\expl}{\mathrm{exp}}
\newcommand{\out}{\mathrm{out}}
\newcommand{\nrmot}[1]{\nrm{#1}_{t}}
\newcommand{\doac}{\mathrm{do}}
\usetikzlibrary{matrix,decorations.pathreplacing,calc}

\newcommand{\MP}{\mathsf{P}^M}
\newcommand{\oMP}{\mathsf{P}^{\oM}}
\newcommand{\oMR}{\mathsf{R}^{\oM}}

\newcommand{\etod}{\textsc{E2D-TA}}
\newcommand{\etodfull}{\textsc{Estimation-to-Decisions with Tempered Aggregation}}
\newcommand{\etodva}{\textsc{E2D-VA}}
\newcommand{\Vovkalg}{Tempered Aggregation}
\newcommand{\ops}{Optimistic Posterior Sampling}
\newcommand{\tPP}{\widetilde{\PP}}
\newcommand{\etap}{\eta_{\mathrm{p}}}
\newcommand{\etar}{\eta_{\mathrm{r}}}
\newcommand{\mops}{\textsc{MOPS}}
\newcommand{\omle}{\textsc{OMLE}}

\newcommand{\dcp}{\operatorname{dcp}}
\newcommand{\dcpha}{\dcp^{h,\alpha}}
\newcommand{\dcpa}{\dcp^{\alpha}}

\newcommand{\eetod}{\textsc{PAC E2D}}
\newcommand{\pexp}{p_{\mathrm{exp}}}
\newcommand{\pout}{p_{\mathrm{out}}}
\newcommand{\hatpout}{\hat{p}_{\mathrm{out}}}
\newcommand{\pac}{{\rm pac}}

\newcommand{\rfec}{\operatorname{rfdec}}
\newcommand{\rfecg}{\operatorname{rfdec}_{\gamma}}
\newcommand{\orfec}{\rfec}
\newcommand{\orfecg}{\orfec_{\gamma}}
\newcommand{\rfalg}{\textsc{Reward-Free E2D}}
\newcommand{\rfetod}{\textsc{Reward-Free E2D}}
\newcommand{\rf}{{\rm rf}}
\newcommand{\rrec}{\operatorname{rrec}}
\newcommand{\rrecg}{\rrec_{\gamma}}
\newcommand{\suboptrf}{\mathbf{SubOpt}^{\mathbf{rf}}}

\def\rfdec{{\rm rfdec}}
\newcommand{\hMP}{\mathsf{P}_{\hM}}
\newcommand{\Pm}{\mathsf{P}}
\newcommand{\Rm}{\mathsf{R}}
\newcommand{\oPm}{\overline{\mathsf{P}}}
\newcommand{\hPm}{\hat{\mathsf{P}}}


\newcommand{\err}{\operatorname{Err}}
\newcommand{\PPs}{\PP^\star}



\newcommand{\piest}{\pi^{\exp}}
\newcommand{\piesth}{\pi^{\exp}_h}
\newcommand{\piesthM}{\piest_{M,h}}

\newcommand{\comp}{\operatorname{comp}}

\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\hmu}{\hat\mu}

\newcommand{\ltwot}[1]{\ltwo{#1}^2}
\newcommand{\dr}{d}
\newcommand{\Rs}{\bR_{\star}}

\newcommand{\ba}{\mathbf{a}}
\renewcommand{\circ}{\diamond}
\newcommand{\Gap}{{\rm Gap}}
\newcommand{\EQ}{{\tt EQ}}

\newcommand{\NE}{{\tt NE}}
\newcommand{\CE}{{\tt CE}}
\newcommand{\CCE}{{\tt CCE}}

\newcommand{\omedec}{\medec}
\newcommand{\MEerr}{\mathbf{Err}_{\mathbf{ME}}}
\newcommand{\mealg}{\textsc{All-Policy Model-Estimation E2D}}
\newcommand{\MEalg}{\textsc{All-Policy Model-Estimation E2D}}

\newcommand{\ME}{\mathrm{me}}
\newcommand{\muout}{\mu_{\out}}
\renewcommand{\opi}{\bar{\pi}}
\newcommand{\DTVPi}[1]{\wdTV^{\Pi}\left(#1\right)}
\newcommand{\mdec}{\operatorname{amdec}}
\newcommand{\medec}{\operatorname{amdec}}
\newcommand{\omdec}{\mdec}
\newcommand{\MDEC}{AMDEC}

\newcommand{\wdTV}{\wt{D}_{\rm RL}}
\newcommand{\wDTV}[1]{\wdTV\left(#1\right)}
\newcommand{\rand}{{\rm rand}}
\newcommand{\DTVPid}[1]{\wdTV^{\Pi^{\det}}\left(#1\right)}
\newcommand{\DTVPir}[1]{\wdTV^{\Pi^{\rand}}\left(#1\right)}

\newcommand{\PbRL}{\rm PbRL}


\newcommand{\Bpara}{B-representation}



\newcommand{\nrmc}[1]{\nrm{#1}_{\star}}
\newcommand{\tauhm}{\tau_{h-1}}
\newcommand{\tauh}{\tau_h}
\newcommand{\thh}{t_{h}}
\newcommand{\thp}{t_{h+1}}

\newcommand{\piexp}{\pi_{\expl}}

\newcommand{\apsr}{\alpha_{\sf psr}}
\newcommand{\arev}{\alpha_{\sf rev}}

\newcommand{\nrmpip}[1]{\nrm{#1}_{\Pi'}}
\newcommand{\nrmpin}[1]{\nrm{#1}_{\Pi}}
\newcommand{\nrmonetwo}[1]{\nrm{#1}_{1, 2}}


\newcommand{\cBHh}{\cB_{H:h}}
\newcommand{\cBHhp}{\cB_{H:h+1}}


\def\oedec{\edec}
\def\orfdec{\rfdec}

\newcommand{\csh}{\sigma}

\newcommand{\inv}{\natural}
\newcommand{\dlr}{d_{\sf trans}}
\newcommand{\dlrh}{d_{{\sf trans},h}}

\newcommand{\cBHhop}{\cB_{H:h}}

\newcommand{\bp}{\mathbf{p}}

\newcommand{\efunc}{f}
\newcommand{\tfunc}{\wt{\efunc}}

\newcommand{\ceth}{\cE_{\theta,h}}
\newcommand{\bqth}{\bds(\tau_{h-1})}

\newcommand{\cEs}{\cE^{\star}}
\newcommand{\pikh}{\pi^k_h}
\newcommand{\pith}{\pi^t_h}

\newcommand{\ocE}{\overline{\cE}}
\newcommand{\obq}{\overline{\bq}}
\newcommand{\obqth}{\obq(\tau_{h-1})}


\newcommand{\stab}{\Lambda_{\sf B}}


\newcommand{\stabs}{$\stab$-stable}
\newcommand{\stabsn}{$\stab$-stablility}

\newcommand{\dum}{\rm dum}

\newcommand{\rb}{R_{\sf B}}
\newcommand{\exend}{{~$\Diamond$}}
\newcommand{\moneone}[1]{\nrm{#1}_{1\to 1}}
\newcommand{\linv}{+}



\newcommand{\rep}{\cG}
\newcommand{\cerr}{\cE}



\newcommand{\taut}{\tau^{(t)}}


\newcommand{\BB}{\mathbf{B}}
\newcommand{\bq}{\mathbf{q}}

\newcommand{\Qh}{\cU_h}
\newcommand{\Qhp}{\cU_{h+1}}
\newcommand{\QAh}{\mathcal{U}_{A,h}}
\newcommand{\QAhp}{\mathcal{U}_{A,h+1}}

\newcommand{\Uone}{\cU_1}
\newcommand{\Uh}{{\cU_h}}
\newcommand{\Uhp}{{\cU_{h+1}}}
\newcommand{\UH}{{\cU_H}}
\newcommand{\UAh}{\mathcal{U}_{A,h}}
\newcommand{\UAhp}{\mathcal{U}_{A,h+1}}
\newcommand{\oUh}{\overline{\cU}_h}
\newcommand{\Uhpp}{{\cU_{h'+1}}}

\newcommand{\nUh}{\abs{\Uh}}
\newcommand{\nUhp}{\abs{\Uhp}}
\newcommand{\nUone}{\abs{\cU_1}}
\newcommand{\nUA}{U_A}
\newcommand{\nUAh}{\abs{\UAh}}
\newcommand{\nUAhp}{\abs{\UAhp}}

\newcommand{\pis}{\pi_\star}
\newcommand{\bbrac}[1]{\Big[#1\Big]}

\newcommand{\og}{\bar{g}}
\newcommand{\Mer}{Model estimation representation}
\newcommand{\mer}{model estimation representation}

\newcommand{\LM}{L}
\newcommand{\qexp}{q_{\exp}}
\newcommand{\qest}{q_{\exp}}


\newcommand{\dimc}{\dim_{\rm c}}


\newcommand{\dtr}{q}

\newcommand{\vgap}{G}

\newcommand{\odimc}{\overline{\dim}_{\rm c}}
\newcommand{\oeluder}{\overline{\mathfrak{e}}}
\newcommand{\ostarn}{\overline{\mathfrak{s}}}

\newcommand{\conv}{\mathrm{conv}}
\newcommand{\normal}[1]{\textsf{N}\paren{#1}}

\newcommand{\wSigma}{\mathbf{\Sigma}}

\newcommand{\belrep}{decouplable representation}
\newcommand{\Belrep}{Decouplable representation}
\newcommand{\mbelrep}{strong decouplable representation}
\newcommand{\mBelrep}{Strong decouplable representation}

\newcommand{\Pia}{\Pi}
\newcommand{\Piab}{\Pi_{\sf Pb}}
\newcommand{\cMpb}{\cM_{\sf Pb}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\decpb}{\pbdec}
\newcommand{\oT}{\overline{\T}}
\newcommand{\Regpb}{\reg^{\bf pb}}
\newcommand{\pbrlalg}{\textsc{Preference-based E2D}}
\newcommand{\pbdec}{{\rm pbdec}}
\newcommand{\opbdec}{\pbdec}
\newcommand{\dT}{d_{\T}}

\newcommand{\onu}{\bar{\nu}}

\newcommand{\ssp}{\mathbb{S}}
\newcommand{\ssps}{\ssp^{\GOAL}}
\newcommand{\ssprf}{\ssp^{\rm rf}}
\newcommand{\sspme}{\ssp^{\rm me}}
\newcommand{\ssppb}{\ssp^{\rm pb}}
\newcommand{\suboptme}{\subopt^{\bf me}}
\newcommand{\suboptpac}{\subopt^{\bf pac}}

\newcommand{\csp}{\mathbb{D}}
\newcommand{\csps}{\csp^{\GOAL}}
\newcommand{\csppb}{\csp^{\rm pb}}

\newcommand{\GOAL}{\mathsf{G}}
\newcommand{\cspreg}{\csp_{\sf reg}}
\newcommand{\csppac}{\csp_{\sf pac}}
\newcommand{\DEC}{\GOAL\!\operatorname{-dec}}
\newcommand{\DECt}{{\rm $\GOAL$-DEC}}
\newcommand{\getod}{$\GOAL$-\textsc{E2D}}
\newcommand{\subopts}{\subopt^{\GOAL}}
\newcommand{\Regs}{\reg^{\GOAL}}

\newcommand{\tbd}[1]{{\color{blue} #1}}

\newcommand{\suboptpb}{\subopt^{\mathbf{pb}}}
\newcommand{\Mtraj}{M_{\sf traj}}
\newcommand{\oMtraj}{\oM_{\sf traj}}
\newcommand{\cMtraj}{\cM_{\sf traj}}
\newcommand{\Cmp}{\C}

\newcommand{\bSigma}{\mathbf{\Sigma}}

\newcommand{\byparts}[2]{&#1\\&#2}
\newcommand{\bypart}[2]{\Big\{&#1\\&~#2\Big\}}

\newcommand{\dimG}{\dim}

